Flavor dependence of unpolarized quark Transverse Momentum Distributions from a global fit

We present an extraction of the unpolarized transverse-momentum-dependent parton distribution and fragmentation functions that takes into account possible differences between quark flavors and final-state hadrons. The extraction is based on experimental measurements from Drell-Yan processes and semi-inclusive deep-inelastic scattering, whose combination is essential to distinguish flavor differences. The analysis is carried out at N$^3$LL accuracy. The extracted flavor-dependent distributions give a very good description of the data ($\chi^2/N_{\rm dat} = 1.08$). The resulting uncertainties take fully into account also the uncertainties in the determination of the corresponding collinear distributions.

==> normalisation.tex <==
\section{Normalization factors for SIDIS}
\label{s:norm_SIDIS}

In Ref.~\cite{Bacchetta:2017gcc} it was demonstrated that TMD factorization at
NLL accuracy is able to successfully reproduce the normalization and shape
of $\hermes$ SIDIS multiplicities and the shape of the available $\compass$
multiplicities. More recently, the $\compass$ collaboration published a reanalysis of their
data~\cite{COMPASS:2017mvk}. The NLL TMD predictions correctly reproduce
normalization and shape of the new data~\cite{Piacenza:2020sst}. However, when
increasing the accuracy to N$^2$LL or higher, the TMD formula severely
underestimates the
measurements~\cite{OsvaldoGonzalez-Hernandez:2019iqj,Piacenza:2020sst} by nearly
constant factors in each bin. Note that tensions between the TMD cross
sections and the associated measurements exist also at large transverse
momentum in SIDIS~\cite{Gonzalez-Hernandez:2018ipj},
DY~\cite{Bacchetta:2019tcu}, and electron-positron annihilation into
two hadrons~\cite{Moffat:2019pci}.

In the present study, as will be shown in Sec.~\ref{s:results}, we confirm that we obtain an
excellent description of both the normalization and shape of the SIDIS
multiplicities at NLL and that the N$^2$LL results are much
smaller. At N$^3$LL the results increase slightly, but they are still far
from the NLL ones and, therefore, from data. At average kinematics of
the $\compass$ measurements, we obtain the following ratios of multiplicities:
\begin{align}
\frac{M_{\rm NLL}}{M_{\rm N^2LL}} &\gtrsim 2,
&
\frac{M_{\rm NLL}}{M_{\rm N^3LL}} &\gtrsim 1.5.
\end{align}

The reason for the difference between the logarithmic orders is almost entirely due to the hard factor in
Eq.~\eqref{e:FUUT_def}~\cite{Collins:2017oxh}. If we look at the explicit expression for
the hard factor\footnote{There are different
definitions for the hard factor in the literature, which are compensated by
different definitions of the matching coefficients $C$ in
Eq.\eqref{e:TMD_matching}. Here we follow the definition of Ref.~\cite{Collins:2017oxh}.} with the standard choice $\mu= Q$
\begin{equation}
{\cal H}^{\rm SIDIS} (Q,Q)=
1 + \frac{\alpha_s(Q)}{4\pi} C_F \bigg(-16+\frac{\pi^2}{3}\bigg),
\end{equation}
we can immediately see that just by introducing ${\cal O}(\alpha_s)$
corrections, at $Q= 2$ GeV with $\alpha_s\approx 0.3$, we reduce
the structure function to about 60\% of its original value.
This change is not compensated by a similar reduction in the
denominator of Eq.~\eqref{e:mult_def}: the differences between the LO and NLO
expressions of the inclusive DIS cross section are typically below 5\% and the
NLO results are actually larger than the LO ones.

If the NLL expression is much larger than the N$^2$LL and N$^3$LL ones, we may suspect that
it should overshoot the data by a factor 1.5 at least.
However, several works before the present one have shown a good
agreement with the data using a parton-model
approach~\cite{Signori:2013mda,Anselmino:2013lza} or
at NLL~\cite{Echevarria:2014xaa,Sun:2014dqm}.
Moreover, the integral of the structure function over
$\qT$ is equal to the value of its Fourier transform at $\bT=0$.
Using any $b^*$ prescription with
$b_{\rm min}=2 e^{-\gamma_E}/Q $, the integral of the NLL expression
by construction corresponds to the LO expression of the collinear
SIDIS structure function, independent of the TMD nonperturbative parameters:\footnote{Note that in the absence of a $b_{\rm min}$ prescription, the integral would vanish.}
\begin{equation}
\begin{split}
\int d^2 \qT \,F_{UU,T}\big( x,z,\modqT,Q \big)
&=
x\, \sum_a e_a^2\, {\cal H}^{\rm SIDIS}(Q,Q)  \bigg(
\hat{f}_1^a(x,\bT^2;Q,Q^2)\,
\hat{D}_1^{a \to h}(z,\bT^2;Q,Q^2)\bigg)\bigg|_{\modbT=0}
\\
&\stackrel{\rm NLL}{=}
x\, \sum_a e_a^2\,
{f}_1^a(x;Q)\,
{D}_1^{a \to h}(z;Q).
\end{split}
\end{equation}

The LO collinear SIDIS predictions are known to describe the data reasonably
well and, if anything, they seem to be lower than the
data~\cite{deFlorian:2007aj,HERMES:2012uyd}. Therefore, the integral of our
NLL expression is in good agreement with data, which also indicates the
absence of a large normalization error.

If the NLL predictions describe the data well and are a factor 2 or 1.5 above
the N$^2$LL and N$^3$LL predictions, we propose to modify the
normalization of the latter to recover a good agreement with data.
An extended discussion of this issue can be
found in Ref.~\cite{Piacenza:2020sst}.
We observe that the integral of the TMD formula, valid at low $\qT$, should
reproduce only part of the full collinear cross section.
The only exception is the order ${\cal O}(\alpha_s^0)$ case, as we have seen
above, since at that order there is no contribution from gluon radiation at
high transverse momentum, beyond the TMD region.

However, at N$^2$LL or higher, in the kinematics of fixed-target SIDIS
experiments, the integral of the TMD region (\textit{i.e.}, the integral of the
so-called $W$ term in the language of Ref.~\cite{Collins:2011zzd}) is much smaller than the
corresponding collinear cross section. The missing contribution to the
integral should be recovered by
the terms in the fixed-order calculation that are not included in the TMD
resummed expression (the so-called $Y$ term).
Ideally, the $Y$ term should be
negligible in the low-$\qT$ region. This is not the case in the
experimental regions under consideration: the $Y$ term is finite but
relatively large, even at $\qT=0$.

If we consider the contribution to the integral of the $W$ term (\textit{i.e.}, the integral of
Eq.~\eqref{e:SIDIS_xsec}), with our $b_{\rm min}$ prescription,
at order $\alpha_s$ we obtain, schematically
\begin{equation}\label{eq:WintDetail}
\int d^2 \qT\,  W \biggr\vert_{{\cal O}(\alpha_s)} =
\sigma_0 \frac{\alpha_s}{4 \pi} \sum_{q} e_q^2 \Bigl[
D_1^{q \to h} \otimes C_{\rm TMD}^{qq}\otimes f_1^{q} +
D_1^{q \to h} \otimes C_{\rm TMD}^{qg}\otimes f_1^{g} +
D_1^{g \to h} \otimes C_{\rm TMD}^{gq}\otimes f_1^{q}
\Bigr](x,z,Q) ,
\end{equation}
where
\begin{equation}
\sigma_0 = \frac{4\pi^2\, \alpha^2\, z^2\, |\qT|}{x\, Q^3} Y_+.
\end{equation}
The double convolution over both $x$ and $z$ is defined as
\begin{equation}
\Bigl[ D_1^{a \to h} \otimes C^{ab}\otimes f_1^{b} \Bigr](x,z,Q) =
\frac{1}{z^2}\int_x^1 \frac{dx'}{x'} \int_z^1\frac{dz'}{z'}
D_1^{a \to h}(z';Q) C^{ab}\Bigl(\frac{x}{x'},\frac{z}{z'} \Bigr) f_1^{b}(x';Q)
\end{equation}
and the $C_{\rm TMD}$ coefficients can be found in
App.~\ref{a:Ccoeff}.

The integral in Eq.~\eqref{eq:WintDetail} should be compared to the collinear expression at the same order (see,
\textit{e.g.}, Ref.~\cite{deFlorian:1997zj})
\begin{equation}
\label{eq:SIDISintNLO}
\begin{split}
\frac{d \sigma^{\text{SIDIS}}}{d x d Q d z} \biggr\vert_{{\cal
O}(\alpha_s)}&=
\sigma_0 \frac{\alpha_s}{4 \pi} \sum_{q} e_q^2 \biggl\{\Bigl[
D_1^{q \to h} \otimes C_{1}^{qq}\otimes f_1^{q} +
D_1^{q \to h} \otimes C_{1}^{qg}\otimes f_1^{g} +
D_1^{g \to h} \otimes C_{1}^{gq}\otimes f_1^{q}
\Bigr](x,z,Q) \\
&\quad +  \frac{1-y}{1+(1-y)^2} \Bigl[
D_1^{q \to h} \otimes C_{L}^{qq}\otimes f_1^{q} +
D_1^{q \to h} \otimes C_{L}^{qg}\otimes f_1^{g} +
D_1^{g \to h} \otimes C_{L}^{gq}\otimes f_1^{q}
\Bigr](x,z,Q)  \biggr\}. \\
\end{split}
\end{equation}
The QCD coefficients $C_{1}^{a b}$
and $C_{L}^{a b}$ are calculated in perturbation theory.
The former can be written as
\begin{align}
\label{e:Ccoeff}
C_{1}^{a b} (x,z;Q,\mu) &= C_{\rm nomix}^{a
b}(x,z,Q,\mu)+ C_{\rm mix}^{a b}(x,z).
\end{align}
The coefficient $C_{\rm nomix}$ is the sum of
all those terms that contain either a
$\delta(1-x)$  or a
$\delta(1-z)$ (or both). Some of these terms are present in
$C_{\rm TMD}$, but not all. This definition holds at all orders in $\alpha_s$.
The $C_L$ matching coefficients, instead, only contain ``mixed'' contributions.
For convenience, we reproduce all coefficients at order $\alpha_s$ in App.~\ref{a:Ccoeff}.

In order to increase the size of the TMD component, we consider the
contribution of all the ``nonmixed'' terms $C_{\rm nomix}$. The reason behind
this choice is that it might be possible to include such terms into a
redefinition of the individual TMDs. Hence, we define
\begin{equation}
\label{e:nomix}
\frac{d \sigma^{\rm nomix}}{d x d Q d z} \biggr\vert_{{\cal
O}(\alpha_s)} =
\sigma_0 \frac{\alpha_s}{4 \pi} \sum_{q} e_q^2 \Bigl[
D_1^{q \to h} \otimes C_{\rm nomix}^{qq}\otimes f_1^{q} +
D_1^{q \to h} \otimes C_{\rm nomix}^{qg}\otimes f_1^{g} +
D_1^{g \to h} \otimes C_{\rm nomix}^{gq}\otimes f_1^{q}
\Bigr](x,z,Q),
\end{equation}
and similarly for higher orders,
and we introduce the following normalization factor:
\begin{equation}
\label{e:norm_SIDIS_def}
\omega(x,z,Q) = \frac{d\sigma^{\rm nomix}}{dx\, dz\, dQ}  \bigg/  \int d^2 \qT\, W  \, .
\end{equation}
We stress that these normalization factors depend only on the collinear PDFs
and FFs, are independent of the parametrization of the nonperturbative
part of the TMDs, and can be computed before performing a fit of
the latter.

At NLL, $\omega(x,z,Q) = 1$.
Beyond NLL, the prefactor becomes larger than one and guarantees that the
integral of the TMD part of the cross section reproduces most of the collinear
cross section, as suggested by the data. On the contrary, without the
enhancement due to the normalization factor, the integral of the TMD part of
the cross section would be too small, requiring a large role of the
high-transverse-momentum tail, which is not observed in the data.
The impact of the normalization factor defined in Eq.~\eqref{e:norm_SIDIS_def}
will be addressed in detail in Sec.~\ref{s:results}.

As a consequence of our procedure,
the theoretical expression for the SIDIS cross section in Eq.~\eqref{e:SIDIS_xsec}
becomes
\begin{equation}
\label{e:sidis_xsec_expr_w_norm}
\frac{d\sigma_\omega^{\text{SIDIS}}}{dx\, dz\, d|\qT|\, dQ} = \omega(x,z,Q)\, \frac{d\sigma^{\text{SIDIS}}}{dx\, dz\, d|\qT|\, dQ} \, .
\end{equation}

